Towards More Robust Natural Language Understanding

Natural Language Understanding (NLU) is a branch of Natural Language Processing (NLP) that uses intelligent computer software to understand texts that encode human knowledge. Recent years have witnessed notable progress across various NLU tasks with deep learning techniques, especially with pretrained language models. Besides proposing more advanced model architectures, constructing more reliable and trustworthy datasets also plays a huge role in improving NLU systems, without which it would be impossible to train a decent NLU model. It's worth noting that the human ability of understanding natural language is flexible and robust. On the contrary, most of existing NLU systems fail to achieve desirable performance on out-of-domain data or struggle on handling challenging items (e.g., inherently ambiguous items, adversarial items) in the real world. Therefore, in order to have NLU models understand human language more effectively, it is expected to prioritize the study on robust natural language understanding. In this thesis, we deem that NLU systems are consisting of two components: NLU models and NLU datasets. As such, we argue that, to achieve robust NLU, the model architecture/training and the dataset are equally important. Specifically, we will focus on three NLU tasks to illustrate the robustness problem in different NLU tasks and our contributions (i.e., novel models and new datasets) to help achieve more robust natural language understanding. Moving forward, the ultimate goal for robust natural language understanding is to build NLU models which can behave humanly. That is, it's expected that robust NLU systems are capable to transfer the knowledge from training corpus to unseen documents more reliably and survive when encountering challenging items even if the system doesn't know a priori of users' inputs.

==> Table/Table_ch2_4.tex <==
\begin{table*}[t!]
\centering

\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccccccccc|c}
\hline
Models & \textbf{What} & \textbf{When} & \textbf{Has} & \textbf{Was} & \textbf{Why} & \textbf{How} & \textbf{Is} & \textbf{Did} & \textbf{Can} & \textbf{Any} & \textbf{Does} &  \textbf{\begin{tabular}[c]{@{}c@{}}KL\\ (Gen$||$GT)\end{tabular}} \\ \hline
NQG & 0.00 & 0.00 & 3.95 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 96.05 & 84.2 \\
+BeamSearch & 29.94 & 0.00 & 5.54 & 0.00 & 0.00 & 0.00 & 1.38 & 0.00 & 0.00 & 0.00 & 63.14 & 45.2 \\
\textbf{+QPP (Ours)} & 8.39 & 0.01 & 25.37 & 4.44 & 0.91 & 0.87 & 9.09 & 0.27 & 4.03 & 12.72 & 33.89 & \textbf{11.0} \\ \hline
NQG++ & 0.09 & 0.00 & 3.53 & 0.00 & 0.00 & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 96.28 & 84.3 \\
+BeamSearch & 44.04 & 0.00 & 0.09 & 0.00 & 0.00 & 0.22 & 2.01 & 0.00 & 0.00 & 0.00 & 53.64 & 66.4 \\
\textbf{+QPP (Ours)} & 8.09 & 0.01 & 25.54 & 4.42 & 0.75 & 0.81 & 9.16 & 0.23 & 4.05 & 12.80 & 34.13 & \textbf{11.2} \\ \hline
BERT-SQG & 0.72 & 0.00 & 6.32 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 92.96 & 74.5 \\
+BeamSearch & 29.31 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 & 25.05 & 0.00 & 0.00 & 0.00 & 45.62 & 47.4  \\
\textbf{+QPP (Ours)} & 8.01 & 0.01 & 25.56 & 4.44 & 0.82 & 0.80 & 9.17 & 0.25 & 4.05 & 12.74 & 34.16 & \textbf{11.2} \\ \hline
GT & 13.80 & 0.01 & 26.73 & 1.94 & 0.63 & 1.16 & 13.24 & 0.14 & 1.31 & 4.11 & 36.93 & - \\ \hline
\end{tabular}%
}
\caption[Distributions of the generated questions and ground truth in emrQA.] {Distributions of the generated questions of different models and the ground truth in the emrQA dataset. QPP: Question Phrase Prediction; KL: Kullback–Leibler divergence. All numbers are percentages.}
\label{tbl_ch2:ques_distribution}
\end{table*}


==> Table/Table_ch4_3.tex <==
\begin{table*}
\centering
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{lrrrrp{0.2cm}rrrr}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{}} & \multicolumn{2}{c}{Dev} & \multicolumn{7}{c}{Test} \\ 
\cmidrule(lr){2-3}
\cmidrule(lr){4-10}
\multicolumn{1}{c}{} & Acc. & F1 & Acc. & F1 && Entail & Neutral & Contradict & Disagree \\
Always 0 & - & -  & - & -  && - & -  & - & - \\
CBOW & 0.40	& 1.47	& 0.55 & 0.22 && 0.00 & 0.00 & 1.43 & 0.56\\
Heuristic & - & -  & - & - && - & -  & - & -\\
Vanilla BERT & 1.14 & 1.17 & 1.75 & 1.81 && 2.96 & 6.90 & 4.42 & 3.65\\ 
joint BERT & 1.31 & 1.44 & 1.49 & 1.80 && 9.36 & 5.40 & 4.40 & 1.83 \\ \midrule
AAs (\texttt{ours}) & 1.41 & 1.44 & 1.28 & 1.42 && 3.70 & 7.48 & 3.12 & 1.94  \\ \bottomrule
\end{tabular}
}
\caption{Standard deviation of baselines and AAs performance on CB dev and test sets.}
\label{tbl_ch4:result_supplementary}
\end{table*}

==> app2.tex <==
\chapter{Important commands defined in {\tt osudissert96}}
\label{allcommands:app}

The following is a list of all commands available in {\tt osudissert96}.


{\baselineskip=15pt
\begin{verbatim}
\author{First Middle Last}
\title{The title of the thesis}
\authordegrees{degree1, degree2}
\unit{Department of Whatever The Name Is}
\degree{Doctor of Philosophy}
\committee{Dissertation}
\advisorname{Name of advisor}  % Possible usage "Prof. Big Dude"
\member{Name of committee member}

\thesis  % this makes it a thesis rather than a dissertation,
         %  similar to the documentclass option [masters] or [ms].

\maketitle

\disscopyright      % or \blankpage

\begin{abstract}
\end{abstract}

\begin{externalabstract}
\end{externalabstract}


\dedication{This is dedicated to \ldots}

\begin{acknowledgements}
\end{acknowledgements}

\begin{vita}
\dateitem{Important Date}{ Why its important}

\begin{publist}
\researchpubs
\pubitem{Bibliography item (from BibTeX?)}

\instructpubs
\pubitem{Bibliography item (from BibTeX?)}
\end{publist}

\begin{fieldsstudy}
\majorfield*        % which uses \unit above
% \majorfield{Your Major Field}
\begin{studieslist}
\studyitem{Topic 1}{Prof.\ 1}
\studyitem{Topic 2}{Prof.\ 2}
\studyitem{Topic 3}{Prof.\ 3}
\end{studieslist}
%% Note:  If there were only one field of study, the following list 
%%        would best be done using the following command:
%%  \onestudy{Only Topic}{Only Professor}
\end{fieldsstudy}

\end{vita}
\end{verbatim}
}

